A clustering-based reinforcement learning approach for tailored personalization of e-Health interventions

Personalization is very powerful in improving the effectiveness of health interventions. Reinforcement learning (RL) algorithms are suitable for learning these tailored interventions from sequential data collected about individuals. However, learning can be very fragile. The time to learn intervention policies is limited as disengagement from the user can occur quickly. Also, in e-Health intervention timing can be crucial before the optimal window passes. We present an approach that learns tailored personalization policies for groups of users by combining RL and clustering. The benefits are two-fold: speeding up the learning to prevent disengagement while maintaining a high level of personalization. Our clustering approach utilizes dynamic time warping to compare user trajectories consisting of states and rewards. We apply online and batch RL to learn policies over clusters of individuals and introduce our self-developed and publicly available simulator for e-Health interventions to evaluate our approach. We compare our methods with an e-Health intervention benchmark. We demonstrate that batch learning outperforms online learning for our setting. Furthermore, our proposed clustering approach for RL finds near-optimal clusterings which lead to significantly better policies in terms of cumulative reward compared to learning a policy per individual or learning one non-personalized policy across all individuals. Our findings also indicate that the learned policies accurately learn to send interventions at the right moments and that the users workout more and at the right times of the day.

==> generative_model.tex <==
\newcounter{mytempeqncnt}

\section{HeartSteps generative model}
\label{heartSteps_generative_model}



\hl{We adopt an existing generative model for e-Health based on the HeartSteps dataset as an additional evaluation of our methods }\cite{dempsey2015randomised}. \hl{The dataset was generated during a 42-day long e-Health intervention trial where the goal was to increase the amount of steps people take everyday by providing interventions in the form of positive messages. These messages for instance suggest going for a walk after a long period of sitting} \cite{zhu2017group}. We briefly describe this generative in this section for the sake of completeness. For a more detailed description of this generative model and the HeartSteps experiment we refer to \cite{zhu2017group,lei2014actor,murphy2016batch}.

\begin{figure*}[]
% ensure that we have normalsize text
\normalsize
% Store the current equation number.
\setcounter{mytempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{0}
\begin{equation}
	\label{eq:generative_model_1}
	\phi_{1}(s_u)(t) \leftarrow \beta_{1}\phi_1(s_u)(t-1) + \xi_{t,1}, \newline
\end{equation}	

\begin{equation}
	\label{eq:generative_model_2}	
	\phi_{2}(s_u)(t) \leftarrow \beta_2\phi_2(s_u)(t-1) +\beta_3*i_{t-1} + \xi_{t,2}, \newline
\end{equation}	
	
\begin{equation}
\begin{aligned}
	\label{eq:generative_model_3}	
	\phi_{3}(s_u)(t) \leftarrow \beta_4\phi_3(s_u)(t-1) + \beta_5*\phi_3(s_u)(t-1)*i_{t-1} + \beta_6*i_{t-1} + \xi_{t,3}, 
\end{aligned}
\end{equation}	
	
\begin{equation}
	\label{eq:generative_model_4}	
	\phi_{n}(s_u)(t) \leftarrow \beta_7\phi_n(s_u)(t-1) + \xi_{t,n},  n = 4,\ldots,p \newline
\end{equation}	

\begin{equation}
\begin{aligned}
\label{eq:generative_model_5}	
r(t) \leftarrow \beta_{14} * \large[\beta_{8} + i_{t} * \large (\beta_{9} + \beta_{10}\phi_{1}(s_u)(t) + \beta_{11}\phi_{2}(s_u)(t) \large) + \beta_{12}\phi_{1}(s_u)(t) - \beta_{13}\phi_{3}(s_u)(t) + \rho_{t} \arge]
\end{aligned}
\end{equation}	


\setcounter{equation}{\value{mytempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}

\subsection{Generative model}
Via a micro-randomized trial \cite{lei2014actor,murphy2016batch}, traces of the form $\langle s, i, r, s^\prime, i^\prime, r^\prime, s^{\prime\prime}, i^{\prime\prime}, r^{\prime\prime}, \ldots \rangle$ were collected from users. Using these experiences, a generative model was developed. In this generative model the initial state is drawn from a predefined Gaussian distribution such that $s_{u}(0) \sim$  $N_{p}\large(0,\Sigma \large)$, where $\Sigma$ is a $p$ x $p$ predefined co-variance matrix. \hl{In this setting, there are two actions where $1$ indicates a positive intervention and $0$ no intervention. Each of these two interventions is selected from a random policy with probability $0.5$. In pour case, there are $3$ numerical states and a numerical reward observable at each time step $t$.} %For more details we refer to} \cite{zhu2017group}. 
For each time-step $t \geq 1$ the state $s_t$ the feature vector representation $\vec{\phi}(s_u)$ for state $s_u$ and the immediate reward are generated using the functions~\ref{eq:generative_model_1}, \ref{eq:generative_model_2}, \ref{eq:generative_model_3}, \ref{eq:generative_model_4}, and \ref{eq:generative_model_5} where $ \beta = \large [\beta_i \large]_{i=1}^{14}$ defines the main parameters for each MDP while $\large [ \xi \large ]_{i=1}^{p} \sim \mathcal{N}(0, \sigma_{s}^{2})$ and $\rho_{t} \sim \mathcal{N}(0, \sigma_{r}^{2})$ are the noise distributions for the state and reward models respectively. 

To generate non-identical experiences for N similar users, N different $\beta$'s need to be created whereby some of these $\beta$'s are close similar to others forming sets. For user $u$ a $\beta$ is assigned following two steps:

\begin{itemize}
\noindent i) Assign user $u$ to basic group $k$ and get the corresponding basic $\beta$ (i.e. $\beta_{k}^{basic}$), \\
\noindent ii) Make each user $u$ within group $k$ different by adding noise $\delta_u \sim \mathcal{N}(0, \sigma_{\beta}\textbf{I}_{14})$ using $\beta_u = \beta_{k}^{basic}$ + $\delta_{u}$ for $i \in [1,2,\ldots,N_k]$. Here $N_k$ defines the number of users in the $k$-th group and $\textbf{I} \in \mathbb R^{14 x 14}$ an identity matrix.\\

\end{itemize}

The exact value chosen the each basic $\beta$ and the parameters of the generative model are discussed in the next section.




==> simulator.tex <==
\section{A simulator for human daily activity}
\label{sec:simulator}

\hl{For the health setting we focus on in this paper, it is difficult to experiment with different RL strategies
% \textbf{MvO: acronyms like RL will solve our space problems we'll definitely have}
and real users, as this requires involving a substantial number of users in a large scale study and gathering too many interaction samples per user. We have therefore decided to build a simulator to experiment with algorithmic settings first. The simulator is created for a realistic setting where users have daily schedules of activities and should be encouraged to conduct certain types of (healthy) activities. In this paper we rely on data from the US time keeping research project to define the underlying parameters of the distributions that drive the order of performed activities for the different profiles we define \cite{hofferth2015american}. Below, we discuss the details of the schedules followed by the interventions and the the possibility to define rewards.}

\subsection{Schedules}

% \textbf{MvO: ik zie veel formuleringen die ingekort kunnen worden, maar dat is voor een latere fase}

We assume that we have $n$ users in our simulator: $\{u_1,\dots,u_n\}$, originating from the set $U$ as defined before. Each of these users can conduct one of $m$ activities at each time point ($\{\varphi_1,\dots,\varphi_m\}$). Time points in our simulator have a discrete step size $\delta t$. Let $\Phi$ denote the possible values of the activity. Example activities are working, sleeping, working out, and eating breakfast. Each user has a unique activity $a \in A$ that is being conducted at a time point $t$ ($activity: A \times T \rightarrow \Phi$). Note that this activity can also be \emph{none}. For each user, a \emph{template} schedule can be specified, which expresses for each activity $\varphi_i$:

\begin{itemize}
\noindent i) an early and late start time
($early\_start(\varphi_i)$ and $late\_start(\varphi_i)$) with multiple instances per day possible,\\
\noindent ii) a minimum and maximum duration of the activity,
($min\_duration(\varphi_i)$ and $max\_duration(\varphi_i)$)\\
\noindent iii) a standard deviation of the duration of the activity(\emph{$sd\_duration(\varphi_i)$}),\\
\noindent iv) a probability per day of performing the activity ($p(\varphi_i, day)$),\\
\noindent v) priorities of other activities over this activity.
\end{itemize}

Using these template schedules, a complete schedule is derived which instantiates %one unique activity% 
activities at each time point, on a per day basis, following Algorithm~\ref{alg:simplanning}.

\texttt{\\}
\texttt{\\}





{\scriptsize
\RestyleAlgo{algoruled} %boxruled
\LinesNumbered
\begin{algorithm}[tbp]
\SetAlgoLined
\algsetup{linenosize=\tiny}
 day = current\_day\ \newline
 \For{\textbf{each} activity $\varphi_i$}{
 $t_{start}(\varphi_i) = rand(early\_start(\varphi_i), late\_start(\varphi_i))$\
 $d(\varphi_i) = Normal(rand(min\_duration(\varphi_i), $\newline  $ max\_duration(\varphi_i)), sd\_duration)$ \newline
 $p(\varphi_i) = p(\varphi_i, day)$\
 }
 t = \emph{start of the day}\ \newline
 active = false\ \newline
 activity\_queue = \{\}\ \newline
 current\_activity = none\ \newline
 \While{$t <$ end of the day}{
 	activity\_queue = clean\_up\_queue(activity\_queue)\
    \For{\textbf{each} activity $a \in A$}{
       	\If{t == $t_{start}(\varphi_i)$}{
        	\If{rand $\leq$ p($\varphi_i$, day)}{
            	activity\_queue = activity\_queue $\cup$ $\varphi_i$\
            }
        }
    }
	current\_activity = select\_from\_queue(activity\_queue)\
    \If{$\neg$ (current\_activity == none)}{
    	active = true\;
    }
    $t = t + \delta t$
}
\caption{Planning activities per day}
\label{alg:simplanning}
\end{algorithm}}

\texttt{\\}

\hl{The algorithm basically uses the ranges for start times and durations of activities to generate actual start times and durations. The start times are drawn randomly from the specified range and the durations are drawn from a normal distribution with the specified mean and standard deviation. It then starts to run a schedule and builds up a queue of activities that are relevant for the current time point (i.e. for which the current time is after the start of the activity and before the end of it). In case of multiple activities, the one already being performed is continued, or in case of a higher priority activity the user switches to that activity. If the queue is empty, the user is not active (or idle) and selects the \emph{none} activity.}





\subsection{Interventions and Rewards}

%\textbf{Dit kan nu een stuk exacter}
% ALI: Added some details to this subsection
Besides performing activities during a day, interventions can also be sent to users. In our system, the set of interventions $I$ contains a binary action as $\{ \mathtt{yes}, \mathtt{no} \}$, representing at each decision moment whether the system sends an intervention or not. \hl{An intervention is a message that tells the user to perform a desired activity $\varphi_i$ (we assume there is only one single desired activity for now which is working out). To decide upon acceptance of a message, users have a profile that expresses the conditions under which the users are willing to accept the intervention. These conditions are expressed by the range of time points during which the users are willing to accept an intervention (e.g. a working person might not accept an intervention when at work).} If a message is sent at the right time %(and when the activity has not been performed yet on that day),% 
and a gap in the schedule is between $t_{plan\_min}$ and $t_{plan\_min} + t_{plan\_duration}$ from the time the message is sent, the activity will be performed. These parameters define a time window in the schedule into which the users will try to fit the desired activity suggested by the intervention. \hl{Rewards can be defined based on acceptance of the message (i.e. the activity is considered part of the queue), commencement of the desired activity, and how long the activity has been performed (e.g. there might be some optimal amount of time spent on the activity). More details on the setting we use for the specific case in this paper are shown in the next section}.


